CADET: Debugging and Fixing Misconfigurations using Counterfactual Reasoning

Modern computing platforms are highly-configurable with thousands of interacting configurations. However, configuring these systems is challenging. Erroneous configurations can cause unexpected non-functional faults. This paper proposes CADET (short for Causal Debugging Toolkit) that enables users to identify, explain, and fix the root cause of non-functional faults early and in a principled fashion. CADET builds a causal model by observing the performance of the system under different configurations. Then, it uses casual path extraction followed by counterfactual reasoning over the causal model to: (a) identify the root causes of non-functional faults, (b) estimate the effects of various configurable parameters on the performance objective(s), and (c) prescribe candidate repairs to the relevant configuration options to fix the non-functional fault. We evaluated CADET on 5 highly-configurable systems deployed on 3 NVIDIA Jetson systems-on-chip. We compare CADET with state-of-the-art configuration optimization and ML-based debugging approaches. The experimental results indicate that CADET can find effective repairs for faults in multiple non-functional properties with (at most) 17% more accuracy, 28% higher gain, and $40\times$ speed-up than other ML-based performance debugging methods. Compared to multi-objective optimization approaches, CADET can find fixes (at most) $9\times$ faster with comparable or better performance gain. Our case study of non-functional faults reported in NVIDIA's forum show that CADET can find $14%$ better repairs than the experts' advice in less than 30 minutes.

==> 11_scalability.tex <==
\section{Scalability of \tool}

To examine the scalability of \tool, we evaluate \tool using the speedtest workload of SQLite database to resolve the latency faults due misconfigurations. SQLite database workloads have higher number of configurable options compared to image, NLP and speech workloads. SQLite workloads exhibit unique compute, memory, data reuse characteristics, and higher memory accesses. As a result, SQLite exposes new system design opportunities to enable efficient inference and much complex interactions between software options. We evaluate \tool on the following two scenarios:

\noindent\paragraph{Increasing number of configuration options.} In the first scenario, we perform a sensitivity analysis of \tool by increasing the size of the configuration space. We start with 47 configuration options which we manually select based on important hardware, kernel configuration options and system events recommended in performance blogs. Then we increase the number of configuration options to 330 by including 206 \texttt{sysctl} kernel configuration options that can tuned without rebooting the system. Finally, we extend the number of configuration options to 530 by including all the system events tracked by \textsc{iperf}. In each cases, we track the time required to discover the causal structure, evaluate the counterfactual queries and resolve a latency fault.  

\noindent\paragraph{Increasing number of configuration options' values.} \tool recommends a fix by computing individual treatment effect to evaluate counterfactual queries. The number of these counterfactual queries depends on the number of values taken by a configuration option. If a configuration option can be set to a large number of values, the number of counterfactual queries needed to be evaluated also increases. To determine the behavior of \tool in such scenarios, we evaluate \tool on by increasing the number of values the hardware and kernel configuration options can be set at while resolving the latency faults in the SQLite speedtest workload. 


==> 1_intro_2.tex <==
% \section{Introduction}

% Modern software systems are highly-configurable \needcitation and are designed to be deployed on heterogeneous hardware environments such as system-on-chip (SoCs), consumer hardware, and high-performance computing platforms. Developers are often unaware of the underlying microarchitectural differences. 
% Consequently, they are prone to incorrectly configuring these systems. Misconfiguration may lead to \textit{non-functional faults}.



% % Consequently, configuring these systems particularly error-prone. Misconfiguration may lead to \textit{non-functional faults}.

% % non-functional faults do not res

% % Together, they comprise the system stack.~\fig{sw_hw_stack} shows a typical system stack wherein the software layers constantly interact with the hardware layers. These interactions are controlled by a number of configurations in the layers.
 

% % Misconfigurations

% % Unexpected interactions between layers result in transient non-functional faults even for systems where such non-functional faults have not been encountered before in other hardware environments. 
% % While these configuration options provide great flexibility, they also present significant challenges for developers who are tasked with optimally configuring these   

% non-functional faults do not resemble a typical software bug where the system crashes or exhibits an obvious misbehavior. Instead, systems that have a non-functional fault are still functional but may either be compromised or may operate with a degraded performance. As a result, as much as 99\% of the non-functional faults that arise due to misconfigurations go unreported~\cite{99ofmisc75:online}. These may have undesirable side-effects such as potential data breaches~\cite{Cloudmis78:online, YoureOne98:online}, high-latency, low throughput, or increased energy consumption~\cite{bryant2003computer, molyneaux2009art, Nistor2015, sanchez2020tandem}. Therefore, it is important to \emph{identify the root cause} of such faults and \emph{fix} early and in principled way.

% % Such non-functional faults happen when the software have been shipped to the customers in situations where customers run such system on a hardware platform where have never been tested before. Such non-functional faults may result in unresponsiveness of the system, excessive usage of energy, heat dissepetations, and in several cases damaging the underlying hardware [complete the list]. Therefore, it is important to \emph{identify the root cause} of such faults and \emph{fix} early and in principled way.

% However, it is extremely challenging to \emph{localize the root cause} of such faults and \emph{find a fix} for them. This is due to the huge configuration space as a result of software hardware interactions. The complex interactions between the configuration options in the software and their interactions with the underlying hardware options results in a combinatorially large space of possible settings. Consequently, inspecting this vast space to identify what caused the non-functional fault can be very challenging. Expecting a developer to understand all these complex interactions and fixing the performance issue is impractical, if not impossible. 


% To alleviate the developers' burden, we developed an approach, called \tool, that enables developers to understand and reason about such non-functional faults. \tool relies on Causal Inference [] and Counterfactual Reasoning [] by creating Structural Causal Models, which acts a rich source of knowledge that characterizes various complex interactions between the software and the hardware layers of a system. \tool (a)~identifies the root cause of non-functional faults, and (b)~estimates the effects of various configurable parameters on the performance, and (c)~prescribes candidate fixes to the relevant configuration options to achieve a performance goal.

% Prior research provides many different performance debugging approaches to help developer to (i) identify the bugs[], (ii) identify root causes of the bugs non-functional faults [], and (iii) find potential fixes []. 
% Statistical Debugging [] uses data to capture faults by generating predicates and reasoning based on statistical methods to identify the most likely root causes of the fault by detecting predicates that are highly ``correlated'' with the failure. In this work, we instead, focus on ``causation'' with the goal to find causally related source of the fault. 


% We evaluated \tool based on the effectiveness in discovering root causes of non-functional faults and finding appropriate fixes in (i) single objective (), (ii) multi-objective (), and (ii) transfer learning scenarios () and compared with (i) statistical debugging and (ii) a popular heuristic approach with 5 large-scale systems. We found that, on average, ....


% \subsubsection**{Contributions} We make the following contributions:
% \begin{itemize}
%     \item 
% \end{itemize}

Modern software systems are highly configurable. They are designed to be seamlessly deployed on (a) variety of hardware platforms, eg., SoCs, cloud systems, etc; and (b) different environmental settings, eg., UAV, autonomous vehicles, robotic systems, etc.
The variability in the software configurations, coupled with the myriad different configuration options offered by each hardware platform makes correctly configuring a software/hardware platform a daunting task that is fraught with errors.
Developers, whose task it is to painstakingly configure these software systems, are often oblivious to the underlying micro-architectural differences of the hardware platform. They therefore tend to misconfigure these systems exposing them to non-functional faults. These non-functional faults are unlike regular software bugs where the system may crash or exhibit an obvious misbehavior. Instead, systems with non-functional faults may still be functional while being compromised or they may operate with a degraded performance.
The sheer number of modalities in which a software may be deployed makes it impossible for one to thoroughly test a software and hardware system in every conceivable deployment. As a result, non-functional faults arise in deployments even if such a fault was never previously observed in the same software or hardware in any other situation. Consequently, as much as 99\% of the non-functional faults go unnoticed/unreported.
While finding and addressing non-functional faults caused by programming errors has drawn considerable attention lately. Identifying and fixing non-functional faults that result from misconfigurations have received less attention. This is because, finding misconfiguration requires one to search over a complex and combinatorially large space. Expecting a software developer to debug a non-functional fault by keeping track of all the complex and intricate relationships is impractical, if not impossible.
One option is to use classical search-based methods or statistical debugging methods. But these lack the mathematical language to express these complex relationships and reason about them effectively. They rely on simple correlation to draw their conclusions which may be incomplete at best, or incorrect at worst.
To solve this problem, we propose a principle approach to identifying and repairing misconfiguration-related-performance-faults can be quite useful for software developers and system administrators.






==> 7_discuss.tex <==
% \section{Discussion}
% \label{sect:discussion}

% \subsection{Limitations of \tool}
% No tool is perfect, \tool is no exception. The efficacy of \tool depends on several factors such as the representativeness of the observational data or the presence of unmeasured confounders that can negatively affect the quality of the causal model. There are instances where the causal model may be incorrect or lack some crucial connections that may result in detecting spurious root causes or recommending incorrect repairs. One promising direction to address this problem would be to use active learning. Specifically, we may refine the causal model with developer assistance. We shall address this in our future work.\tool uses a query engine to translate common user queries into counterfactual statements. It could benefit greatly from a formal translation framework (in the form of a DSL) that can convert any user-provided query into a meaningful counterfactual statement. This shall be addressed in our future work.

% \subsection{Threats to Validity}
% \label{sect:threats}
% Typical to other approaches,  biases can affect the final results. Therefore, one has to consider the following issues before deriving any conclusions based on this work: 

% \subsubsection*{Evaluation Bias} In RQ1, RQ2, and RQ3, we have compared the performance of \tool with other approaches to conclude using the metrics described in ~(\tion{metrics}). While those results are true, it is possible to draw slightly different conclusions using other evaluation metrics. We aim to explore this in future research. 
% \subsubsection*{Construct  Validity} We made several engineering decisions in this paper, (e.g.) choice of causal graph discovery algorithms (in our case NOTEARS and FCI), number of observational data, causal effect estimation approaches (semi-parametric and non-parametric), number of repeats in measurement to handle measurement noise, etc. While these decisions were made by suggestions from the literature, we admit that other constructs can derive different conclusions.

% \subsubsection*{External  Validity} For this approach, we selected a diverse set of software systems of different applications and resource-constrained hardware systems. We also selected some configuration options from each layer of the systems stack to detect the root cause of non-functional faults under complex interactions. However, there is a possibility to obtain slightly different results with different performance bugs or configuration options in different systems. Therefore, one has to be particularly careful when generalizing our results to other subject systems. Even though we tried to run our experiments on a diverse subject systems variety from different domains, we do not claim that these results generalize beyond the systems explored in this study. However, we make our scripts and dataset available for reproducibility.

==> 8_threats.tex <==
\section{Threats to Validity}
\label{sect:threats}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> colors.tex <==
\sethlcolor{lightgray}
\definecolor{pink}{RGB}{252,145,149}
\definecolor{lightpink}{RGB}{252,145,149}
\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgray}{gray}{0.6}
\definecolor{Gray}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\definecolor{Blue}{RGB}{0,29,193}
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45} 
\definecolor{pink}{RGB}{231,95,110}
\definecolor{lightergray}{rgb}{0.85, 0.85, 0.85}
\definecolor{lightestgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{codebg}{HTML}{F4F4F4}

% ---- Grays ----
\definecolor{gray05}{gray}{0.95}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray90}{gray}{0.10}


==> figures/DAG_tie_breaking.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[][FCI (PAG).]{\includegraphics[width=0.3\linewidth]{fig__fci_sample_1.pdf}\label{fig:fci_samp}}
    %
    ~
    %
    \subfloat[][NOTEARS (DAG).]{\includegraphics[width=0.3\linewidth]{fig__notears_sample_1.pdf}\label{fig:notears_samp}}
    %
    ~
    %
    \subfloat[][Final ADMG.]{\includegraphics[width=0.3\linewidth]{fig__DAG_sample.pdf}\label{fig:dag_samp}}
    \caption{\small Resolving ties between FCI and NOTEARS.}
    \label{fig:ties}
\end{figure}

==> figures/cauper_samp.tex <==
\begin{figure}[t!]
    \setlength{\belowcaptionskip}{-1em}
    \centering

    % \subfloat[][Using \tool for debugging.]{
        \includegraphics[width=\linewidth]{fig__cauper_samp.pdf}\label{fig:cauper_samp}
        % }
    %
    %
    %
    % \subfloat[][Using \texttt{iperf} and \texttt{top} command line profilers for debugging.]{\includegraphics[width=0.5\linewidth]{fig__iperf.pdf}\label{fig:iperf_samp}}
    
    \caption{\small A simplified causal model used in \tool. \protect\edgeone~shows the causal paths between configurations and between configurations and non-functional properties like latency, energy consumption, \etc. The numbers represent the magnitude of causal effect.}
    % \caption{\small Mechanisms to debug non-functional faults. Here, (a) shows a simplified causal model \tool builds to debug non-functional faults, \eg, when debugging for latency, the \red{$\boldsymbol{\longrightarrow}$} shows the causal paths from the configurations to latency and the numbers represent the magnitude of causal effect; (b) shows an sample \texttt{iperf} (for network load information) and \texttt{top} (for system load information) trace used to pinpoint and fix a real-world performance bug~\cite{HighCPUu7:online}}
    \label{fig:sample}
\end{figure}

==> figures/objectives_overlap.tex <==
\begin{wrapfigure}[11]{R}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig__venn.pdf}
    \caption{\small Summary of \protect\tab{perf_faults_summary}. Numbers in {\color[HTML]{CC3333} \bfseries red} indicate cases with more than one non-functional faults.}
    \label{fig:objectives_overlap}
\end{wrapfigure}

==> listings/listing__cauper.tex <==
\begin{figure}[t!]
    
    \begin{minipage}{\linewidth}
            \algcauper
        %     \caption{\small \tool framework.}
        \end{minipage}
        \\[-1em]
    %     \begin{minipage}{\linewidth}
    %             \algquery
    %             % \caption{\small Generating interventions.}
    % \end{minipage}
\end{figure}

% \begin{figure*}
%     \subfloat[][\tool]{
%         \begin{minipage}{0.5\linewidth}
%             \algcauper
%         \end{minipage}}
%     \subfloat[][Counterfactual query generation]{
%         \begin{minipage}{0.5\linewidth}
%             \algquery
%         \end{minipage}}
% \end{figure*}

==> spacing.tex <==
% \setlength{\belowcaptionskip}{-10pt}
% \setlength{\floatsep}{10pt}
% \setlength{\textfloatsep}{10pt}
% \setlength{\dbltextfloatsep}{10pt}
% \setlength{\fboxsep}{.2pt}
\begin{comment}
% % \setlength{\multicolsep}{2.0pt}% 50% of original values


% % \DeclarePairedDelimiter\abs{\lvert}{\rvert}%
% ----- Change the spacing before and after equations globally -----
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{2pt}
  \setlength\belowdisplayskip{2pt}
  \setlength\abovedisplayshortskip{2pt}
  \setlength\belowdisplayshortskip{2pt}
}
\makeatother

% % \makeatletter
% % \def\thm@space@setup{%
% %   \thm@preskip=0cm plus 0cm minus 0cm
% %   \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
% % }
% % \makeatother

% % \newtheorem{definition}{Definition}

\titleformat{\subsubsection*}[runin]{\bf\normalsize}{\thesubsubsection*}{0em}{}[\xspace\mbox{}]
\titlespacing*{\subsubsection*}{0pt}{0ex plus 0ex minus 0ex}{0pt}

% % \titlespacing*{\section}{5pt}{0.3\baselineskip}{0.3\baselineskip}
% % \titlespacing*{\subsection}{3pt}{0.5\baselineskip}{0.5\baselineskip}
\titleformat*{\subsubsection}{\em\xspace}
% % \titlespacing*{\subsubsection}{2pt}{0.1\baselineskip}{0.1\baselineskip}
\end{comment}

%\titleformat{\subsubsection*}[runin]{\bf\normalsize}{\thesubsubsection*}{0em}{}[\xspace\mbox{}]
% \titlespacing*{\subsubsection*}{0pt}{0ex plus 0ex minus 0ex}{0pt}
% \setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*}%, wide=0pt}
% \setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*}%, wide=0pt}
% \titlespacing*{\subsection}{3pt}{0.75\baselineskip}{0.75\baselineskip}


==> tables/config_options.tex <==
\begin{table}[h]
\caption{\small Configurations options by each layer.}
\small 
\resizebox{\linewidth}{!}{\begin{tabular}[t]{p{0.35\linewidth}|p{0.3\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}}
 
\centering
Configuration options& & Layer&\\
\midrule
\multicolumn{5}{c}{Workload}\\
\cmidrule(lr){1-5}\\ 
&\multicolumn{4}{c}{DNN}\\
\cmidrule(lr){2-5}\\
Memory growth & 0, 0.1, 0.5&\\
Logical devices & 10, 50\\ 
\cmidrule(lr){2-5}\\
&\multicolumn{4}{c}{SQLite}\\
\cmidrule(lr){2-5}\\
Cache size & 0, 0.1, 0.5&\\
Buffer size & 10, 50\\ 
Synchronous & 0, 1 \\
Journal mode & Memory, Disk \\
Temporary store & Memory, Disk \\

\cmidrule(lr){2-5}\\
&\multicolumn{4}{c}{x264}\\
\cmidrule(lr){2-5}\\
CRF & 0, 0.1, 0.5&\\
Preset & 10, 50\\
Bit rate & 10,100\\
Latency & 1,2 \\
\hline 
\multicolumn{5}{c}{OS/Kernel}\\
\cmidrule{1-5}\\
Scheduler policy& CFP, NOOP\\
Swappiness&10, 60, 100\\
Dirty background ratio&10, 80\\
Dirty ratio& 5, 50\\
Sched child runs first & 0, 1 \\
Drop caches & 0, 1, 2, 3\\
Cache pressure & 1, 100, 500 \\

\hline
\multicolumn{5}{c}{Hardware}\\
\cmidrule{1-5}\\
& \multicolumn{1}{l}{\nano}&\multicolumn{1}{l}{\txone} & \multicolumn{1}{l}{\txtwo} & \multicolumn{1}{l}{\xavier}\\
\cmidrule{2-2}\cmidrule{3-3}\cmidrule{4-4}\cmidrule{5-5}\\
Active CPUs&1 - 4&1 - 4&1 - 4&1 - 4\\
CPU freq. (GHz)&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\
GPU freq. (GHz)& 0.1 - 1.3&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\
EMC freq. (GHz)&0.1 - 1.8&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\

\bottomrule
\end{tabular}}
\label{tab:configurations}
\end{table}%}

==> tables/dag_edge_types.tex <==
% \begin{table}[tbp!]
%     \caption{\small How FCI transforms a fully connected dense graph $(G)$ to a skeleton graph $(S)$ and to Partial DAG (PAG). %Note, the nodes Y and Z are \textit{not} independent when they are not conditioned on other variables (denoted by $\dagger$); but when conditioned on X, they become independent (denoted by $\ddagger$), thus the edge $Y\text{---}Z$ is removed in the skeleton. 
%     }
%     \label{tab:fci_example}
%     \resizebox*{\linewidth}{!}{
%     \begin{tabular}{crcc}
%         \hlineB{2}
%     Dense G           & Independence & Skeleton $(S)$   & Partial DAG $(PAG)$      \bigstrut\\\hlineB{2}

%     \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_full.pdf}}} 
%     & $X\notindependent Y$     & \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_pruned.pdf}}} & \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_dir.pdf}}} \bigstrut\\
%                       & $X\notindependent Z$     &         &          \bigstrut\\
%                       & $X\independent W$     &         &          \bigstrut\\
%                       & $Y\notindependent Z^{\dagger}$     &     &              \bigstrut\\
%                       & $Y\notindependent W$     &               &    \bigstrut\\
%                       & $Z\notindependent W$     &              &     \bigstrut\\
%                       & $Y\independent Z~|~X^{\ddagger}$   &  & \\\hlineB{2}               
%     \end{tabular}}
% \end{table}
    

    

==> tables/manual_study.tex <==
% \begin{figure}[t!]
%     \setlength{\belowcaptionskip}{-1em}
%     \centering
%     \subfloat[t][]{    
%     \resizebox{0.45\linewidth}{!}{\adjustbox{valign=b}{%
%     \begin{tabular}{lrrrr}
%         \hlineB{2}
%         Type& \rotatebox{90}{\txone~} & \rotatebox{90}{\txtwo} & \rotatebox{90}{\xavier~} & \rotatebox{90}{Total}\bigstrut\\\hlineB{2}
%         Latency & 6 & 9 & {5} & \cellcolor{gray05}20 \bigstrut[t]\\
%         Energy & 6 & 4 & {8} & \cellcolor{gray05}17 \\
%         Thermal & 5 & 2 & {2} & \cellcolor{gray05}9 \bigstrut[b]\\
%         \rowcolor{gray05} Total & 17 & 15 & 15 & \cellcolor{gray12} 47 \bigstrut\\ \hlineB{2}
%     \end{tabular}%
%     \label{tab:perf_faults_count}
%     }
%     }
%     }~
%     \subfloat[t][]{
%         \includegraphics[width=0.45\linewidth, valign=b]{fig__venn.pdf}
%         \label{fig:perf_faults_venn}
%     }    
% \caption{\small non-functional faults in reported in NVIDIA Jetson\textsuperscript (gathered from NVIDIA developer forum). (a) Distribution across hardware, (b) Distribution across fault type ({\color[HTML]{CC3333} \bfseries red} indicate cases with multiple non-functional fault types).}
% \label{tab:perf_faults_summary}
% \end{figure}

==> tables/rq1_gain.tex <==
\begin{table}[t!]
    \centering
    \caption{\small (RQ1) Performance gain (\eq{gain}) up on applying repairs prescribed by respective approaches. Larger gains (in \colorbox[HTML]{C9E7BF}{green}) are considered better. \tool achieves better $\Delta_{gain}$ overall.}
    \label{tab:rq1_2}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ll|lll|lll|lll|}
     &  & \multicolumn{3}{c|}{TX1} & \multicolumn{3}{c|}{TX2} & \multicolumn{3}{c|}{\xavier} \bigstrut\\ \clineB{3-11}{2} 
     & Software & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Latency}} & DNN Image & \cellcolor[HTML]{C9E7BF}78 & 75 & 71 & \cellcolor[HTML]{C9E7BF}75 & 53 & 46 & \cellcolor[HTML]{C9E7BF}89 & \cellcolor[HTML]{C9E7BF}89 & 61 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}86 & 70 & 60 & \cellcolor[HTML]{C9E7BF}79 & 51 & 34 & \cellcolor[HTML]{C9E7BF}89 & 67 & 80 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}76 & 72 & 66 & \cellcolor[HTML]{C9E7BF}94 & 76 & 54 & \cellcolor[HTML]{C9E7BF}90 & 77 & 64 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}29 & 27 & 10 & \cellcolor[HTML]{C9E7BF}28 & 13 & 5 & \cellcolor[HTML]{C9E7BF}35 & \cellcolor[HTML]{C9E7BF}35 & 20 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}32 & 20 & 10 & \cellcolor[HTML]{C9E7BF}32 & 10 & 11 & \cellcolor[HTML]{C9E7BF}29 & 11 & 13 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Energy}} & DNN Image & \cellcolor[HTML]{C9E7BF}77 & 41 & 18 & \cellcolor[HTML]{C9E7BF}89 & 51 & 30 & \cellcolor[HTML]{C9E7BF}79 & 53 & 41 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}76 & 51 & 9 & 67 & \cellcolor[HTML]{C9E7BF}77 & 40 & \cellcolor[HTML]{C9E7BF}69 & 47 & 30 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}71 & 42 & 19 & \cellcolor[HTML]{C9E7BF}76 & 66 & 42 & \cellcolor[HTML]{C9E7BF}76 & 47 & 35 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}32 & 16 & 9 & \cellcolor[HTML]{C9E7BF}24 & 13 & 6 & \cellcolor[HTML]{C9E7BF}32 & 20 & 5 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}25 & 13 & 12 & \cellcolor[HTML]{C9E7BF}23 & 10 & 7 & \cellcolor[HTML]{C9E7BF}26 & 19 & 6 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Thermals}} & DNN Image & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 3 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 3 & \cellcolor[HTML]{C9E7BF}8 & 1 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}4 & 3 & 3 & \cellcolor[HTML]{C9E7BF}7 & 5 & 2 & \cellcolor[HTML]{C9E7BF}3 & 2 & 3 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}7 & 3 & 4 & \cellcolor[HTML]{C9E7BF}7 & 4 & 2 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}8 & 2 & 1 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 1 & \cellcolor[HTML]{C9E7BF}8 & 3 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}6 & 5 & 2 & \cellcolor[HTML]{C9E7BF}5 & 3 & 2 & \cellcolor[HTML]{C9E7BF}3 & 1 & 1 \bigstrut\\ \hlineB{2}
    \end{tabular}%
    }
    \end{table}

==> tables/rq2.tex <==
%  \begin{table}[]
%      \centering
%      \caption{\small (RQ2) Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults. Cells highlighted in \colorbox{blue!10}{green} indicate better performance and \colorbox[HTML]{FFCCC9}{red} indicate cases where the performance drops. Note: the results are reported for two kinds of faults in TX2: (1) faults in both latency and energy; and (2) faults in latency, energy, and heat dissipation.}
%      \label{tab:rq2}
%      \resizebox{\linewidth}{!}{
%      \begin{tabular}{ll|rr|rr|rr|}
%       &  & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \multicolumn{1}{r|}{\rotatebox{90}{Default}} \bigstrut\\ \cline{3-8} 
%       & Software & \multicolumn{2}{r|}{Accuracy} & \multicolumn{2}{r|}{Recall} & \multicolumn{2}{r|}{Precision} \bigstrut\\ \hlineB{2}
%      \multicolumn{1}{l|}{\multirow{6.5}{*}{Latency and Energy}} & DNN Image & \cellcolor{blue!10}59 & 51 & \cellcolor{blue!10}44 & 35 & \cellcolor{blue!10}65 & 56 \bigstrut\\
%      \multicolumn{1}{l|}{} & DNN   Speech & \cellcolor{blue!10}66 & 49 & \cellcolor{blue!10}51 & 43 & \cellcolor{blue!10}74 & 64 \bigstrut\\
%      \multicolumn{1}{l|}{} & DNN NLP & \cellcolor{blue!10}56 & 53 & \cellcolor{blue!10}42 & \cellcolor{blue!10}42 & \cellcolor{blue!10}66 & 61 \bigstrut\\
%      \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}51 & 48 & \cellcolor{blue!10}55 & 33 & \cellcolor{blue!10}64 & 56 \bigstrut\\
%      \multicolumn{1}{l|}{} & SQLite & \cellcolor{blue!10}60 & 51 & \cellcolor{blue!10}57 & 37 & \cellcolor{blue!10}72 & 57 \bigstrut\\ \hlineB{2}
%      \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \cellcolor{blue!10}67 & 59 & \cellcolor{blue!10}69 & 60 & \cellcolor{blue!10}64 & 60 \bigstrut\\
%      \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}68 & 62 & \cellcolor{blue!10}79 & 56 & \cellcolor{blue!10}68 & 58 \bigstrut\\
%      \multicolumn{1}{l|}{} & SQLite & \cellcolor{blue!10}79 & 63 & \cellcolor{blue!10}70 & 57 & \cellcolor{blue!10}84 & 63 \bigstrut\\ \hlineB{2}\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}\bigstrut\\[-0.4cm]\hlineB{2}
%      \multicolumn{1}{l}{\multirow{9.5}{*}{Latency and Energy}} & \multicolumn{1}{r|}{$\Delta_{gain}\longrightarrow$} & \multicolumn{2}{c|}{{Latency}} & \multicolumn{2}{c|}{{Energy}} & \multicolumn{2}{c|}{{Thermals}} \bigstrut\\ \hlineB{2} 
    
%      \multicolumn{1}{l|}{} & DNN Image & \cellcolor{blue!10}52 & \multicolumn{1}{l|}{33} & \multicolumn{1}{l}{\cellcolor{blue!10}37} & \multicolumn{1}{l|}{22} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & DNN   Speech & \multicolumn{1}{l}{\cellcolor{blue!10}60} & \multicolumn{1}{l|}{25} & \multicolumn{1}{l}{\cellcolor{blue!10}54} & \multicolumn{1}{l|}{17} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & DNN NLP & \multicolumn{1}{l}{\cellcolor{blue!10}49} & \multicolumn{1}{l|}{30} & \multicolumn{1}{l}{\cellcolor{blue!10}51} & \multicolumn{1}{l|}{17} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & x264 & \multicolumn{1}{l}{\cellcolor{blue!10}23} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{\cellcolor{blue!10}12} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-2} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & SQLite & \multicolumn{1}{l}{\cellcolor{blue!10}9} & \multicolumn{1}{l|}{6} & \multicolumn{1}{l}{\cellcolor{blue!10}11} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\ \hlineB{2}
    
%      \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \multicolumn{1}{l}{\cellcolor{blue!10}54} & \multicolumn{1}{l|}{29} & \multicolumn{1}{l}{\cellcolor{blue!10}31} & \multicolumn{1}{l|}{16} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{1} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & x264 & \multicolumn{1}{l}{\cellcolor{blue!10}18} & \multicolumn{1}{l|}{1} & \multicolumn{1}{l}{\cellcolor{blue!10}10} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\
   
%      \multicolumn{1}{l|}{} & SQLite & \multicolumn{1}{l}{\cellcolor{blue!10}6} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l}{\cellcolor{blue!10}7} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{0} \bigstrut\\ \hlineB{2}
%      \end{tabular}
%      }
%      \end{table}

\begin{table*}[]
    \centering
    \caption{\small {Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults: \textit{Energy, Latency}; and \textit{Energy, Latency, Heat}. Cells highlighted in \colorbox{blue!10}{green} indicate improvement over faults and \colorbox[HTML]{FFCCC9}{red} indicate deterioration. \tool achieves better performance overall and is much faster. Note: the results are reported for NVIDIA Jetson TX2.}}
    \label{tab:rq2}
    \footnotesize
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}l@{}ll|llll|llll|llll|llll|llll|llll|ll|}
            \clineB{4-29}{2}
            &  &  & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{Precision} & \multicolumn{4}{c|}{Recall} & \multicolumn{4}{c|}{Gain (Latency)} & \multicolumn{4}{c|}{Gain (Energy)} & \multicolumn{4}{c|}{Gain (Heat)} & \multicolumn{2}{c|}{Time$^\dagger$} \bigstrut\\ \clineB{4-29}{2}
            % &  &  &  &  &  &  &  &  & \\[-1em]\clineB{4-29}{2} 
            
            &  &  & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{Others} \\ \clineB{4-29}{2}
            
            \multicolumn{1}{l}{}&\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\[-0.9em]\hlineB{2}

            & \multicolumn{1}{l|}{} & Image & \cellcolor{blue!10}\textbf{77} & 54 & 55 & 65 & \cellcolor{blue!10}\textbf{73} & 53 & 54 & 62 & \cellcolor{blue!10}\textbf{80} & 59 & 59 & 62 & \cellcolor{blue!10}\textbf{83} & 53 & 61 & 65 & \cellcolor{blue!10}\textbf{70} & 38 & 46 & 44 & \cellcolor{blue!10}\textbf{3} & 0 & 0 & 0 & \cellcolor{blue!10}\textbf{0.6} & 4 \\
            & \multicolumn{1}{l|}{} & NLP & \cellcolor{blue!10}\textbf{70} & 51 & 56 & 65 & \cellcolor{blue!10}\textbf{71} & 42 & 56 & 63 & \cellcolor{blue!10}\textbf{66} & 59 & 62 & 65 & \cellcolor{blue!10}\textbf{68} & 53 & 59 & 61 & \cellcolor{blue!10}\textbf{60} & 41 & 27 & 48 & \cellcolor{blue!10}\textbf{5} & 0 & 0 & 1 & \cellcolor{blue!10}\textbf{0.2} & 4 \\
            & \multicolumn{1}{l|}{} & Speech & \cellcolor{blue!10}\textbf{74} & 50 & 61 & 65 & \cellcolor{blue!10}\textbf{68} & 44 & 53 & 62 & \cellcolor{blue!10}\textbf{79} & 51 & 59 & 64 & \cellcolor{blue!10}\textbf{82} & 55 & 55 & 62 & \cellcolor{blue!10}\textbf{66} & 43 & 43 & 41 & \cellcolor{blue!10}\textbf{4} & \cellcolor[HTML]{FFCCC9}-2 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.7} & 4 \\
            & \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}\textbf{83} & 54 & 55 & 66 & \cellcolor{blue!10}\textbf{81} & 50 & 54 & 57 & \cellcolor{blue!10}\textbf{77} & 63 & 62 & 61 & \cellcolor{blue!10}\textbf{15} & 2 & 4 & 6 & \cellcolor{blue!10}\textbf{13} & 4 & 6 & 4 & \cellcolor{blue!10}\textbf{2} & \cellcolor[HTML]{FFCCC9}-3 & \cellcolor[HTML]{FFCCC9}-1 & 0 & \cellcolor{blue!10}\textbf{1.2} & 4 \\
           \multirow{-5}{*}{\rotatebox{90}{Energy +}} & \multicolumn{1}{l|}{\multirow{-5}{*}{\rotatebox{90}{Latency}}} & SQLite & \cellcolor{blue!10}\textbf{84} & 51 & 58 & 68 & \cellcolor{blue!10}\textbf{80} & 43 & 55 & 62 & \cellcolor{blue!10}\textbf{84} & 57 & 63 & 65 & \cellcolor{blue!10}\textbf{11} & 5 & 4 & 5 & \cellcolor{blue!10}\textbf{14} & 3 & 8 & 8 & \cellcolor{blue!10}\textbf{2} & \cellcolor[HTML]{FFCCC9}-2 & 0 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.5} & 4 \\ \hlineB{2}

           \multicolumn{1}{l}{}&\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\[-0.95em]\hlineB{2}

            & \multicolumn{1}{l|}{} & Image & \cellcolor{blue!10}\textbf{76} & 57 & 48 & 66 & \cellcolor{blue!10}\textbf{68} & 61 & 57 & 61 & \cellcolor{blue!10}\textbf{81} & 53 & 46 & 70 & \cellcolor{blue!10}\textbf{62} & 33 & 30 & 42 & \cellcolor{blue!10}\textbf{52} & 23 & 18 & 24 & \cellcolor{blue!10}\textbf{4} & 1 & 0 & 0 & \cellcolor{blue!10}\textbf{0.1} & 4 \\
            & \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}\textbf{80} & 59 & 47 & 54 & \cellcolor{blue!10}\textbf{76} & 61 & 56 & 63 & \cellcolor{blue!10}\textbf{81} & 56 & 46 & 51 & \cellcolor{blue!10}\textbf{12} & 2 & 1 & 2 & \cellcolor{blue!10}\textbf{15} & 4 & 2 & 4 & \cellcolor{blue!10}\textbf{4} & 1 & 0 & 1 & \cellcolor{blue!10}\textbf{0.1} & 4 \\
           \multirow{-3}{*}{\rotatebox{90}{All}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\rotatebox{90}{Three}}} & SQLite & \cellcolor{blue!10}\textbf{73} & 56 & 51 & 53 & \cellcolor{blue!10}\textbf{68} & 59 & 56 & 60 & \cellcolor{blue!10}\textbf{78} & 54 & 45 & 51 & \cellcolor{blue!10}\textbf{12} & 1 & 1 & 4 & \cellcolor{blue!10}\textbf{8} & 4 & 2 & 5 & \cellcolor{blue!10}\textbf{1} & 1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.1} & 4 \\ \hlineB{2}
           \multicolumn{10}{l}{$^\dagger$ Wallclock time in hours}\bigstrut
           \end{tabular}
    }
\end{table*}
    

==> tables/rq3.tex <==
\begin{table}[]
    \caption{\small (RQ3) Transferring causal models across hardware platforms. Default uses the configurations from NIVIDA's Jetpack SDK. Update 10\% uses 10\% of the available budget to sample observations from the target environment to update the causal model. Remodel uses 100\% of the allocated budget to generate new samples and build a causal model from scratch on the target hardware.}
    \label{tab:rq3}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll|rrr|rrr|rrr|rrr}
        \hlineB{2}
        \multicolumn{14}{c}{TX1 (source) $\longrightarrow$ TX2 (target)} \bigstrut\\ \hlineB{2}

        & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Accuracy} & \multicolumn{3}{c|}{Recall} & \multicolumn{3}{c|}{Precision} & \multicolumn{3}{c}{$\Delta_{gain}$} 
        
        \bigstrut\\ \clineB{3-14}{2} 
        
        &  Software & \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~} & \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}& \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}& \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}\bigstrut\\ \hlineB{2}       

    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Latency}}} & Image & 52 & 78 & 88 & 70 & 79 & 86 & 46 & 78 & 91 & 46 & 66 & 74 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 55 & 67 & 76 & 57 & 79 & 75 & 45 & 57 & 81 & 33 & 65 & 79 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 45 & 59 & 64 & 56 & 79 & 62 & 49 & 56 & 74 & 54 & 82 & 94 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 47 & 75 & 83 & 70 & 79 & 82 & 58 & 67 & 85 & 5 & 19 & 28 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 59 & 68 & 80 & 68 & 76 & 78 & 52 & 64 & 84 & 10 & 22 & 31 \bigstrut\\ \hlineB{2}
    \multicolumn{14}{c}{TX2 (source) $\longrightarrow$ XAVIER (target)} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Energy}}} & Image & 53 & 70 & 84 & 48 & 71 & 86 & 51 & 59 & 78 & 30 & 81 & 88 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 50 & 71 & 77 & 53 & 75 & 80 & 49 & 68 & 74 & 40 & 59 & 67 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 57 & 66 & 73 & 45 & 74 & 70 & 43 & 53 & 77 & 42 & 69 & 76 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 54 & 70 & 79 & 46 & 79 & 77 & 42 & 65 & 83 & 6 & 13 & 24 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 45 & 65 & 82 & 48 & 79 & 70 & 47 & 63 & 81 & 7 & 16 & 23 \bigstrut\\ \hlineB{2}
    \multicolumn{14}{c}{Xavier (source) $\longrightarrow$ TX1 (target)} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Thermals}}} & Image & 53 & 62 & 65 & 69 & 61 & 80 & 58 & 64 & 64 & 3 & 4 & 4 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 55 & 60 & 69 & 69 & 59 & 76 & 52 & 63 & 69 & 3 & 3 & 4 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 57 & 58 & 66 & 69 & 63 & 81 & 53 & 63 & 63 & 3 & 5 & 7 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 51 & 58 & 68 & 73 & 51 & 76 & 54 & 71 & 66 & 1 & 4 & 7 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 54 & 58 & 70 & 70 & 62 & 75 & 48 & 66 & 66 & 1 & 6 & 6 \bigstrut\\ \hlineB{2}
    \end{tabular}
    }
    \end{table}

==> tables/study_systems.tex <==
% \begin{table}[t!]
%     \caption{\small Overview of workloads used in our experiments.}
%     \label{tab:perf_faults_summary}
%     \centering
%     \resizebox{0.9\linewidth}{!}{%
%     \begin{tabular}{lrrrr}
%     \hlineB{2}
%     Workload & Domain & $d$ & $|C|$ & $|H|$\\\hlineB{2}
%     Xception & Image recognition (DNN) & 13 & 1408 & 4 \\
%     BERT & Natural language processing (DNN) & 13 & 1376 & 4 \\
%     DeepSpeech & Speech recognition (DNN) & 13 & 1128 & 4 \\
%     SQLite & Database & 17 & 1684 & 3 \\
%     x264& Video encoding & 19 & 1843 & 3 \\ 
    
%     \end{tabular}%
% }
% \end{table}

\begin{table}[]
    \centering
    \caption{\small (RQ2) Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults. Cells highlighted in \colorbox[HTML]{C9E7BF}{green} indicate better performance and \colorbox[HTML]{FFCCC9}{red} indicate cases where the performance drops. Note: the results are reported for two kinds of faults in TX2: (1) faults in both latency and energy; and (2) faults in latency, energy, and heat dissipation.}
    \label{tab:rq2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|r|rrrrr|}
     &  & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \multicolumn{1}{r|}{\rotatebox{90}{Default}} \bigstrut\\ \cline{3-8} 
     & Software & \multicolumn{2}{r|}{Accuracy} & \multicolumn{2}{r|}{Recall} & \multicolumn{2}{r|}{Precision} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{6.5}{*}{Latency and Energy}} & DNN Image & \cellcolor[HTML]{C9E7BF}59 & 51 & \cellcolor[HTML]{C9E7BF}44 & 35 & \cellcolor[HTML]{C9E7BF}65 & 56 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN   Speech & \cellcolor[HTML]{C9E7BF}66 & 49 & \cellcolor[HTML]{C9E7BF}51 & 43 & \cellcolor[HTML]{C9E7BF}74 & 64 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}56 & 53 & \cellcolor[HTML]{C9E7BF}42 & \cellcolor[HTML]{C9E7BF}42 & \cellcolor[HTML]{C9E7BF}66 & 61 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}51 & 48 & \cellcolor[HTML]{C9E7BF}55 & 33 & \cellcolor[HTML]{C9E7BF}64 & 56 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}60 & 51 & \cellcolor[HTML]{C9E7BF}57 & 37 & \cellcolor[HTML]{C9E7BF}72 & 57 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \cellcolor[HTML]{C9E7BF}67 & 59 & \cellcolor[HTML]{C9E7BF}69 & 60 & \cellcolor[HTML]{C9E7BF}64 & 60 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}68 & 62 & \cellcolor[HTML]{C9E7BF}79 & 56 & \cellcolor[HTML]{C9E7BF}68 & 58 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}79 & 63 & \cellcolor[HTML]{C9E7BF}70 & 57 & \cellcolor[HTML]{C9E7BF}84 & 63 \bigstrut\\ \hlineB{2}\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}\bigstrut\\[-0.4cm]\hlineB{2}
    \multicolumn{1}{l}{\multirow{9.5}{*}{Latency and Energy}} & \multicolumn{1}{r|}{$\Delta_{gain}\longrightarrow$} & \multicolumn{2}{c|}{{Latency}} & \multicolumn{2}{c|}{{Energy}} & \multicolumn{2}{c|}{{Thermals}} \bigstrut\\ \hlineB{2} 
    
    \end{tabular}
    }
    \end{table}


==> tables/systems.tex <==
\begin{table}
 \caption{\small Summary of hardware systems, software systems, and configuration options. Note: Some configuration options do not apply to certain software systems (we highlight these with $\cdot$). We also include 17 non-intervenable systems events.}
 \label{tab:systems}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}ll|ccc|@{}c|c@{}}
        \hlineB{2}
       

        & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Deep Neural Network} & \multicolumn{1}{c|}{Database} & \multicolumn{1}{c}{Encoder}
        
        \\ \clineB{3-7}{1.5}
        
        &  Config Options &{\rotatebox[origin=c]{0}{Image}~\textsuperscript{\red{a}}} & {\rotatebox[origin=c]{0}{NLP}}~\textsuperscript{\red{b}} & {\rotatebox[origin=c]{0}{Speech}}~\textsuperscript{\red{c}} & SQLite &x264  \\ \hlineB{2}       

    \multicolumn{1}{l|}{\multirow{4}{-1em}{\rotatebox{90}{Hardware}}} & Cpu cores  & {\footnotesize\color{gray50} $\checkmark$} & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}  \\
    \multicolumn{1}{l|}{} & EMC freq      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}     \\
    \multicolumn{1}{l|}{} & CPU freq                                      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & GPU freq                                    & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}     \\ \hlineB{2}
   
    \multicolumn{1}{l|}{\multirow{8}{*}{\rotatebox{90}{OS/Kernel}}} & Scheduler policy                                     & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Sched child runs first                                  & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Sched rt runtime                     & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$} \\
    \multicolumn{1}{l|}{} & Drop caches                                           & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Dirty background ratio                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}         & {\footnotesize\color{gray50} $\checkmark$}   \\ 
     \multicolumn{1}{l|}{} & Dirty ratio                                         & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}  \\
          \multicolumn{1}{l|}{}&VFS cache pressure                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}                      \\
      \multicolumn{1}{l|}{}&Swappiness                                      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}  \\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{9}{*}{\rotatebox{90}{Application}}} & GPU Memory growth                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {$\cdot$} & {$\cdot$} \\
    
    \multicolumn{1}{l|}{} & Clear session                & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {$\cdot$} & {$\cdot$} \\
               
     \multicolumn{1}{l|}{}& Preset                       & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}                   \\ 
    \multicolumn{1}{l|}{} & Filter& {\footnotesize\color{gray50} $\cdot$}             & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}\\ 
    
     \multicolumn{1}{l|}{} & Bit rate    & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}               \\
    \multicolumn{1}{l|}{} & Pragma journal mode                        & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                   \\ 
    \multicolumn{1}{l|}{} & Pragma synchronous          & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}  \\ 
     \multicolumn{1}{l|}{}& Pragma cache size                     & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                    \\ 
    
    \multicolumn{1}{l|}{}  &Pragma page size                       & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                  \\ \hlineB{2}  
    \end{tabular}
    }
    {\scriptsize \textsuperscript{\red{a}} Xception+CIFAR10~\cite{chollet2017xception, cifar10} \textsuperscript{\red{b}} BERT+IMDb~\cite{devlin2018bert, maas-EtAl:2011:ACL-HLT2011} \textsuperscript{\red{c}} DeepSpeech~\cite{hannun2014deep}}
    \end{table}
    

==> tex/RQ1.tex <==
% \begin{figure*}[tbp!]
%     \begin{minipage}{\linewidth}
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/readelf.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/nm.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/size.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/strip.pdf}
%         \end{subfigure}
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/legend.pdf}
%         \end{subfigure}
%     \end{minipage}\\
%     \begin{minipage}{\linewidth}
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/objdump.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/libjpeg.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/libxml.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/mupdf.pdf}
%         \end{subfigure}~%
%         \begin{subfigure}[t]{0.195\linewidth}
%             \includegraphics[width=\linewidth]{figures/RQ1/harfbuzz.pdf}
%         \end{subfigure}
%     \end{minipage}
%     \caption{\small {\small Total edge coverage comparison of \tool with other state-of-the-art fuzzers each run for 24 hours.}}
%     \label{fig:RQ1_charts}
% \end{figure*}

\begin{figure*}[tbp!]
    \includegraphics[width=0.82\linewidth]{figures/rq1.pdf}
    \vspace{-3mm}
    \caption{\small {\small Edge coverage over 24 hours of fuzzing by \tool and other state-of-the-art fuzzers. 
   % The data was gathered using \texttt{afl-clang-fast}. Similar conclusion can be drawn from \texttt{afl-gcc}.
    }}
    \label{fig:RQ1_charts}
\end{figure*}

